A Quantum-Inspired Analysis of Human Disambiguation Processes

Formal languages are essential for computer programming and are constructed to be easily processed by computers. In contrast, natural languages are much more challenging and instigated the field of Natural Language Processing (NLP). One major obstacle is the ubiquity of ambiguities. Recent advances in NLP have led to the development of large language models, which can resolve ambiguities with high accuracy. At the same time, quantum computers have gained much attention in recent years as they can solve some computational problems faster than classical computers. This new computing paradigm has reached the fields of machine learning and NLP, where hybrid classical-quantum learning algorithms have emerged. However, more research is needed to identify which NLP tasks could benefit from a genuine quantum advantage. In this thesis, we applied formalisms arising from foundational quantum mechanics, such as contextuality and causality, to study ambiguities arising from linguistics. By doing so, we also reproduced psycholinguistic results relating to the human disambiguation process. These results were subsequently used to predict human behaviour and outperformed current NLP methods.

==> Background/QIT/QC.tex <==
\begin{itemize}
    \item The different formalisms for quantum computations. (MBQC and the gate-based model)
    \item The standard algorithms (phase estimation, amplitude amplification)
    \item Where does the speed-up come from
    \item NISQ and heuristic algorithms (and why we need them, i.e. quantum systems are not stable, so small number of qubits, and a lot of decoherence = noise)
\end{itemize}

==> Background/QIT/outside.tex <==
\begin{itemize}
    \item Quantum Psychology etc.
    \item Quantum NLP and ML (the mainstream approaches)
    \item Monoidal categories and DisCoCat
\end{itemize}

==> ImpactStatement.tex <==
\paragraph{}Large Language Models (LLMs) are used in everyday life nowadays, especially with applications such as ChatGPT. These LLMs are data-hungry, which creates reproducibility and environmental issues. Furthermore, they act as a ``black box’’, and whether they learn the same language features as humans is unclear.

\paragraph{}In recent years, research in quantum information theory has led to machine learning algorithms using near-term quantum computers. These advances offer the possibility of using quantum computers for NLP purposes. However, results about quantum advantages in these near-term learning algorithms are yet to be found. 

\paragraph{} This project aimed to address some of these issues. The impact of this work is mainly academic, where our contributions spanned multiple fields, including Natural Language Processing, Quantum Computing, and Linguistics. The project also has the potential to develop a new generation of more cognitively plausible learning algorithms.

\section*{Human and quantum processes}

\paragraph{}This project aimed to bring forward similarities between linguistic and physical phenomena using a shared mathematical language. Drawing a parallel between linguistic and quantum mechanical concepts may help identify which NLP tasks could benefit from quantum resources. The non-determinism of natural language ambiguities notably offered a promising place to start.

\paragraph{}Regarding cognitive plausibility issues, we adopted a foundational approach and looked at human disambiguating strategies. The framework identified essential structures of the disambiguation process, aligning with psycholinguistic theories. We then used the established structure to simulate some disambiguation processes using near-term quantum computers.

\section*{An interdisciplinary project}

\paragraph{}This project involved elements from various research fields, including psycholinguistics, artificial intelligence, and quantum computing, and opened new avenues for research in each of them.

\paragraph{Natural Language Processing} This project provides an alternative, more cognitively plausible, and transparent approach to NLP. By exploiting the structure of the human disambiguation process and the computational power of quantum systems, we produced a learning algorithm that delivers results even with a small training dataset.%\red{compare to LLM}

\paragraph{Quantum Computing}In this work, we provide a strategy for finding applications of quantum computing in areas that are, on the surface, unrelated to quantum mechanics. For instance, this project provided the first instance of quantum(-like) contextuality in linguistic data, where contextuality is a fundamental distinction between classical and quantum statistics.

\paragraph{Linguistics}By introducing the mathematical tools from quantum physics, we provide new tools to study linguistic phenomena and cognitive processes. Using these mathematical frameworks, we can create new models of cognitive processes that are, by design, easy to simulate using quantum resources.

